Controllability of Acoustic Waves by Point Sources: Reachable States and Stable Reconstruction

We study the terminal controllability of the three-dimensional acoustic wave equation driven by finitely many fixed point sources, with zero initial data and time-dependent amplitudes supported in a finite interval. Although finitely many fixed sources cannot control the whole energy space, we establish the following results: (i) For source amplitudes in the first-order Sobolev space in time, the terminal state has finite energy if and only if all amplitudes vanish at both endpoints of the control interval. (ii) We derive an exact frequency-domain identity for the terminal energy involving a Gram matrix whose diagonal entries are one and whose off-diagonal entries are given by the sinc function, depending on frequency and source separation. (iii) For every positive control time, the terminal control operator is bounded below and is an isomorphism onto its closed reachable range, which has infinite codimension even among states satisfying the finite-propagation support condition. (iv) We establish a necessary and sufficient radiation-field criterion for reachability, provide stable reconstruction of the unique controls, and characterize the best approximation of non-reachable targets. The optimal coercivity constant equals one before the shortest source travel time. At long times, it decays as the inverse square of the control time for two sources and as the inverse fourth power for three equally spaced collinear sources. We also obtain upper bounds for general configurations and illustrate the theoretical results through reproducible Galerkin computations.

==> numerics/convergence_table.tex <==
\begin{tabular}{lrrrrr}
\hline
Configuration & $cT/d$ & $N=40$ & $N=80$ & $N=160$ & $N=320$ \\
\hline
Two sources & 2 & 0.6816901 & 0.6816901 & 0.6816901 & 0.6816901 \\
Two sources & 10 & 0.0575299 & 0.0575252 & 0.0575246 & 0.0575245 \\
Two sources & 20 & 0.0154432 & 0.0154379 & 0.0154372 & 0.0154371 \\
Tetrahedron & 1.5 & 0.7829119 & 0.7829052 & 0.7829044 & 0.7829043 \\
Collinear triple & 10 & 0.0044883 & 0.0044862 & 0.0044860 & 0.0044859 \\
Collinear triple & 20 & 0.0003170 & 0.0003163 & 0.0003163 & 0.0003162 \\
\hline
\end{tabular}

